Both Spatial and Frequency Cues Contribute to High-Fidelity Image Inpainting

Deep generative approaches have obtained great success in image inpainting recently. However, most generative inpainting networks suffer from either over-smooth results or aliasing artifacts. The former lacks high-frequency details, while the latter lacks semantic structure. To address this issue, we propose an effective Frequency-Spatial Complementary Network (FSCN) by exploiting rich semantic information in both spatial and frequency domains. Specifically, we introduce an extra Frequency Branch and Frequency Loss on the spatial-based network to impose direct supervision on the frequency information, and propose a Frequency-Spatial Cross-Attention Block (FSCAB) to fuse multi-domain features and combine the corresponding characteristics. With our FSCAB, the inpainting network is capable of capturing frequency information and preserving visual consistency simultaneously. Extensive quantitative and qualitative experiments demonstrate that our inpainting network can effectively achieve superior results, outperforming previous state-of-the-art approaches with significantly fewer parameters and less computation cost. The code will be released soon.

==> tables/rst.tex <==
% celeba
% \begin{table}[!t]
% \renewcommand\arraystretch{1.5}
% \huge

% \center
% \definecolor{darkgreen}{RGB}{40,240,123}
% \begin{center}
% \caption{Quantitative evaluation of state-of-the-art approaches with out model on the CelebA-HQ dataset~\cite{celeba-hq}. \textcolor{red}{Red color} denotes decrease and \textcolor{darkgreen}{green color} denotes improvement compared to our model (presented in the first row). }
% \label{tab:celeb}
% \vspace{-2mm}

%  \resizebox{1.0\columnwidth}{!}{
% \begin{tabular}{l |ccc |ccc |ccc}
% %\begin{tabular}{llccccccccc}
% \hline
% \multirow{2}{*}{Method}   &  \multicolumn{3}{c|}{Thin} &  \multicolumn{3}{c|}{Medium} &  \multicolumn{3}{c}{Thick}   \\

% \cline{2-10} 
%  &FID\downarrow & LPIPS\downarrow & SSIM\uparrow    &FID\downarrow & LPIPS\downarrow & SSIM\uparrow  &FID\downarrow & LPIPS\downarrow & SSIM\uparrow  \\
% \hline

% Ours  &4.6739 &0.0762 &0.9247 &4.9603 &0.0766 &0.9162 &5.4149 &0.0897 &0.8971
% \\ \hline


% \multirow{2}{*}{LaMa}  &5.7965 &0.0825 &0.9208 &5.2425 &0.0792 &0.9141 &5.5395 &0.0924 &0.8942 \\
% &  \textcolor{red}{24.02\%} &\textcolor{red}{8.27\%} &\textcolor{red}{0.42\%} &\textcolor{red}{5.69\%} &\textcolor{red}{3.39\%} &\textcolor{red}{0.23\%} &\textcolor{red}{2.30\%} &\textcolor{red}{3.01\%} &\textcolor{red}{0.32\%} \\ \hline


% \multirow{2}{*}{Wavefill}  &5.2502 &0.079 &0.9207 &5.4269 &0.0815 &0.9096 &5.6187 &0.0963 &0.8889 \\
% &   \textcolor{red}{12.33\%} &\textcolor{red}{3.67\%} &\textcolor{red}{0.43\%} &\textcolor{red}{9.41\%} &\textcolor{red}{6.40\%} &\textcolor{red}{0.72\%} &\textcolor{red}{3.76\%} &\textcolor{red}{7.36\%} &\textcolor{red}{0.91\%} \\ \hline


% \multirow{2}{*}{DMFN}  &7.8631 &0.1055 &0.9070 &6.2192 &0.0888 &0.9062 &6.9401 &0.1041 &0.8839 \\
% &   \textcolor{red}{68.23\%} &\textcolor{red}{38.45\%} &\textcolor{red}{1.91\%} &\textcolor{red}{25.38\%} &\textcolor{red}{15.93\%} &\textcolor{red}{1.09\%} &\textcolor{red}{28.17\%} &\textcolor{red}{16.05\%} &\textcolor{red}{1.47\%} \\ \hline

% \multirow{2}{*}{MADF}  &6.9000 &0.0858 &0.9166 &10.2428 &0.1027 &0.8992 &16.4815 &0.1331 &0.8706 \\
% &  \textcolor{red}{47.63\%} &\textcolor{red}{12.60\%} &\textcolor{red}{0.88\%} &\textcolor{red}{106.50\%} &\textcolor{red}{34.07\%} &\textcolor{red}{1.86\%} &\textcolor{red}{204.37\%} &\textcolor{red}{48.38\%} &\textcolor{red}{2.95\%} \\ \hline

% \multirow{2}{*}{GC}  &11.1879 &0.1295 &0.8964 &8.1926 &0.1063 &0.8954 &9.9133 &0.1213 &0.8690 \\
% &   \textcolor{red}{139.37\%} &\textcolor{red}{69.95\%} &\textcolor{red}{3.06\%} &\textcolor{red}{65.16\%} &\textcolor{red}{38.77\%} &\textcolor{red}{2.27\%} &\textcolor{red}{83.07\%} &\textcolor{red}{35.23\%} &\textcolor{red}{3.13\%} \\ \hline

% \multirow{2}{*}{EC}  &7.0074 &0.0921 &0.9124 &6.1678 &0.0919 &0.9033 &6.9193 &0.1107 &0.8783  \\
% &  \textcolor{red}{49.29\%} &\textcolor{red}{20.87\%} &\textcolor{red}{1.33\%} &\textcolor{red}{24.34\%} &\textcolor{red}{19.97\%} &\textcolor{red}{1.41\%} &\textcolor{red}{27.78\%} &\textcolor{red}{23.41\%} &\textcolor{red}{2.10\%} \\\hline         

% \end{tabular}
%  }
% \end{center}
% %\vspace{-5mm}
% \end{table}


% place
% \definecolor{darkgreen}{RGB}{40,240,123}
% \begin{table}[!t]
% \renewcommand\arraystretch{1.5}
% \huge

% \center
% \begin{center}
% \caption{Quantitative evaluation of state-of-the-art approaches with our model on the Places dataset~\cite{place}. \textcolor{red}{Red color} denotes decrease and \textcolor{darkgreen}{green color} denotes improvement compared to our model (presented in the first row).}
% \label{tab:place}
% \vspace{-2mm}

%  \resizebox{1.0\columnwidth}{!}{
% \begin{tabular}{l |ccc |ccc |ccc }
% %\begin{tabular}{llccccccccc}
% \hline
% \multirow{2}{*}{Method}  &  \multicolumn{3}{c|}{Thin} &  \multicolumn{3}{c|}{Medium} &  \multicolumn{3}{c}{Thick}   \\

% \cline{2-10} 
% & FID\downarrow & LPIPs\downarrow & SSIM\uparrow    &FID\downarrow & LPIPS\downarrow & SSIM\uparrow  &FID\downarrow & LPIPS\downarrow & SSIM\uparrow  \\
% \hline

% Ours  &0.5436 &0.0807 &0.9184 &1.1555 &0.1077 &0.8860 &2.1703 &0.1316 &0.8640
% \\ \hline


% \multirow{2}{*}{LaMa}  &0.6380 &0.0905 &0.9153 &1.3152 &0.1121 &0.8857 &2.2150 &0.1334 &0.8669 \\
% &   \textcolor{red}{17.37\%} &\textcolor{red}{12.14\%} &\textcolor{red}{0.34\%} &\textcolor{red}{13.82\%} &\textcolor{red}{4.09\%} &\textcolor{red}{0.03\%} &\textcolor{red}{2.06\%} &\textcolor{red}{1.37\%} &\textcolor{darkgreen}{0.34\%} \\ \hline

% \multirow{2}{*}{MAT} &0.6298 &0.0951 &0.9033 &1.2386 &0.1216 &0.8676 &1.8765 &0.1430 &0.8428 \\
% &   \textcolor{red}{15.86\%} &\textcolor{red}{17.84\%} &\textcolor{red}{1.64\%} &\textcolor{red}{7.19\%} &\textcolor{red}{12.91\%} &\textcolor{red}{2.08\%} &\textcolor{darkgreen}{13.54\%} &\textcolor{red}{8.66\%} &\textcolor{red}{2.45\%} \\ \hline

% % \multirow{2}{*}{Wavefill}  &0.9794 &0.0994 &0.9075 &1.1959 &0.2828 &0.6473 &1.3204 &0.3679 &0.5467 \\
% %   & \textcolor{red}{80.17\%} &\textcolor{red}{23.17\%} &\textcolor{red}{1.19\%} &\textcolor{red}{3.50\%} &\textcolor{red}{162.58\%} &\textcolor{red}{26.94\%} &\textcolor{red}{39.16\%} &\textcolor{red}{179.56\%} &\textcolor{red}{36.72\%} \\ \hline

% \multirow{2}{*}{MADF}  &0.5787 &0.0857 &0.9140 &1.6844 &0.1145 &0.8796 &3.7856 &0.1377 &0.8560 \\
%   & \textcolor{red}{6.46\%} &\textcolor{red}{6.20\%} &\textcolor{red}{0.48\%} &\textcolor{red}{45.77\%} &\textcolor{red}{6.31\%} &\textcolor{red}{0.72\%} &\textcolor{red}{74.43\%} &\textcolor{red}{4.64\%} &\textcolor{red}{0.93\%} \\ \hline

% \multirow{2}{*}{Deepfillv2}  &1.0668 &0.1044 &0.9061 &2.7125 &0.1300 &0.8688 &5.2606 &0.1541 &0.8391 \\
%  & \textcolor{red}{96.25\%} &\textcolor{red}{29.37\%} &\textcolor{red}{1.34\%} &\textcolor{red}{134.75\%} &\textcolor{red}{20.71\%} &\textcolor{red}{1.94\%} &\textcolor{red}{142.39\%} &\textcolor{red}{17.10\%} &\textcolor{red}{2.88\%} \\ \hline

% \multirow{2}{*}{EdgeConnect}  &1.3542 &0.1110 &0.9347 &3.6796 &0.1347 &0.8720 &8.5293 &0.1588 &0.8492 \\
% &  \textcolor{red}{149.12\%} &\textcolor{red}{37.55\%} &\textcolor{darkgreen}{1.77\%} &\textcolor{red}{218.44\%} &\textcolor{red}{25.16\%} &\textcolor{red}{1.58\%} &\textcolor{red}{293.00\%} &\textcolor{red}{20.67\%} &\textcolor{red}{1.71\%} \\\hline         
% \end{tabular}
%  }
% \end{center}

% %\vspace{-5mm}
% \end{table}



\definecolor{darkgreen}{RGB}{40,240,123}
\begin{table*}[!htb]
\renewcommand\arraystretch{1.5}
\Huge 



\center
\begin{center}
\caption{Quantitative evaluation of state-of-the-art approaches with our model on the Places dataset~\cite{place}. \textcolor{red}{Red color} denotes decrease and \textcolor{darkgreen}{green color} denotes improvement compared to our model (presented in the first row).}
\label{tab:rst}
%\vspace{-2mm}

 \resizebox{\textwidth}{!}{
\begin{tabular}{l |ccc |ccc |ccc |ccc |ccc |ccc}
\hline
\multirow{3}{*}{Method}  &\multicolumn{9}{c|}{CelebA-HQ(256\times256)} &\multicolumn{9}{c}{Places(512\times512)}\\

\cline{2-19}
& \multicolumn{3}{c|}{Thin} &  \multicolumn{3}{c|}{Medium} &  \multicolumn{3}{c|}{Thick} &  \multicolumn{3}{c|}{Thin} &  \multicolumn{3}{c|}{Medium} &  \multicolumn{3}{c}{Thick}   \\

\cline{2-19}
 &FID\downarrow & LPIPS\downarrow & SSIM\uparrow    &FID\downarrow & LPIPS\downarrow & SSIM\uparrow  &FID\downarrow & LPIPS\downarrow & SSIM\uparrow  &FID\downarrow & LPIPS\downarrow & SSIM\uparrow    &FID\downarrow & LPIPS\downarrow & SSIM\uparrow  &FID\downarrow & LPIPS\downarrow & SSIM\uparrow \\
\hline

Ours  &4.6739 &0.0762 &0.9247 &4.9603 &0.0766 &0.9162 &5.4149 &0.0897&0.8971 

&0.5436 &0.0807 &0.9184 &1.1555 &0.1077 &0.8860 &2.1703 &0.1316 &0.8640
\\
\hline

\multirow{2}{*}{LaMa}  &5.7965 &0.0825 &0.9208 &5.2425 &0.0792 &0.9141 &5.5395 &0.0924 &0.8942 

&0.6380 &0.0905 &0.9153 &1.3152 &0.1121 &0.8857 &2.2150 &0.1334 &0.8669\\

  & \textcolor{red}{24.02\%} &\textcolor{red}{8.27\%} &\textcolor{red}{0.425\%} &\textcolor{red}{5.69\%} &\textcolor{red}{3.39\%} &\textcolor{red}{0.23\%} &\textcolor{red}{2.30\%} &\textcolor{red}{3.01\%} &\textcolor{red}{0.32\%} 

&\textcolor{red}{17.37\%} &\textcolor{red}{12.14\%} &\textcolor{red}{0.34\%} &\textcolor{red}{13.82\%} &\textcolor{red}{4.09\%} &\textcolor{red}{0.03\%} &\textcolor{red}{2.06\%} &\textcolor{red}{1.37\%} &\textcolor{darkgreen}{0.34\%}
\\ \hline


\multirow{2}{*}{DMFN} &7.8631 &0.1055 &0.9070 &6.2192 &0.0888 &0.9062 &6.9401 &0.1041 &0.8839 
 &\multirow{2}{*}{-} &\multirow{2}{*}{-} &\multirow{2}{*}{-} &\multirow{2}{*}{-} &\multirow{2}{*}{-} &\multirow{2}{*}{-} &\multirow{2}{*}{-} &\multirow{2}{*}{-} &\multirow{2}{*}{-} \\ 

 &\textcolor{red}{68.23\%} &\textcolor{red}{38.45\%} 
&\textcolor{red}{1.91\%} &\textcolor{red}{25.38\%} &\textcolor{red}{15.93\%} &\textcolor{red}{1.09\%} &\textcolor{red}{28.17\%} &\textcolor{red}{16.05\%} &\textcolor{red}{1.47\%}
& & & & & & & & & &
\hline


\multirow{2}{*}{Wavefill} &5.2502 &0.079 &0.9207 &5.4269 &0.0815 &0.9096 &5.6187 &0.0963 &0.8889 
&\multirow{2}{*}{-} &\multirow{2}{*}{-} &\multirow{2}{*}{-} &\multirow{2}{*}{-} &\multirow{2}{*}{-} &\multirow{2}{*}{-} &\multirow{2}{*}{-} &\multirow{2}{*}{-} &\multirow{2}{*}{-} \\
& \textcolor{red}{80.17\%} &\textcolor{red}{23.17\%} &\textcolor{red}{1.19\%} &\textcolor{red}{3.50\%} &\textcolor{red}{162.58\%} &\textcolor{red}{26.94\%} &\textcolor{red}{39.16\%} &\textcolor{red}{179.56\%} &\textcolor{red}{36.72\%} & & & & & & & & & \\ \hline

\multirow{2}{*}{MAT} 
&\multirow{2}{*}{-} &\multirow{2}{*}{-} &\multirow{2}{*}{-} &\multirow{2}{*}{-} &\multirow{2}{*}{-} &\multirow{2}{*}{-} &\multirow{2}{*}{-} &\multirow{2}{*}{-} &\multirow{2}{*}{-}
&0.6298 &0.0951 &0.9033 &1.2386 &0.1216 &0.8676 &1.8765 &0.1430 &0.8428 \\

 & & & & & & & & &
&\textcolor{red}{15.86\%} &\textcolor{red}{17.84\%} &\textcolor{red}{1.64\%} &\textcolor{red}{7.19\%} &\textcolor{red}{12.91\%} &\textcolor{red}{2.08\%} &\textcolor{darkgreen}{13.54\%} &\textcolor{red}{8.66\%} &\textcolor{red}{2.45\%} \\ \hline


% \multirow{2}{*}{Wavefill} &5.2502 &0.079 &0.9207 &5.4269 &0.0815 &0.9096 &5.6187 &0.0963 &0.8889 

% &0.9794 &0.0994 &0.9075 &1.1959 &0.2828 &0.6473 &1.3204 &0.3679 &0.5467
% \\

%   & \textcolor{red}{12.33\%} &\textcolor{red}{3.67\%} &\textcolor{red}{0.43\%} &\textcolor{red}{9.41\%} &\textcolor{red}{6.40\%} &\textcolor{red}{0.72\%} &\textcolor{red}{3.76\%} &\textcolor{red}{7.36\%} &\textcolor{red}{0.91\%} 

% & \textcolor{red}{80.17\%} &\textcolor{red}{23.17\%} &\textcolor{red}{1.19\%} &\textcolor{red}{3.50\%} &\textcolor{red}{162.58\%} &\textcolor{red}{26.94\%} &\textcolor{red}{39.16\%} &\textcolor{red}{179.56\%} &\textcolor{red}{36.72\%}
% \\ \hline



\multirow{2}{*}{MADF} &6.900 &0.0858 &0.9166 &10.2428 &0.1027 &0.8992 &16.4815 &0.1331 &0.8706 

&0.5787 &0.0857 &0.9140 &1.6844 &0.1145 &0.8796 &3.7856 &0.1377 &0.8560
\\

  & \textcolor{red}{47.63\%} &\textcolor{red}{12.60\%} &\textcolor{red}{0.88\%} &\textcolor{red}{106.50\%} &\textcolor{red}{34.07\%} &\textcolor{red}{1.86\%} &\textcolor{red}{204.37\%} &\textcolor{red}{48.38\%} &\textcolor{red}{2.85\%} 

& \textcolor{red}{6.46\%} &\textcolor{red}{6.20\%} &\textcolor{red}{0.48\%} &\textcolor{red}{45.77\%} &\textcolor{red}{6.31\%} &\textcolor{red}{0.72\%} &\textcolor{red}{74.43\%} &\textcolor{red}{4.64\%} &\textcolor{red}{0.93\%}
\\ \hline



\multirow{2}{*}{Deepfillv2}  &11.1879 &0.1295 &0.8964 &8.1926 &0.1063 &0.8954 &9.9133 &0.1213 &0.8690 

 &1.0668 &0.1044 &0.9061 &2.7125 &0.1300 &0.8688 &5.2606 &0.1541 &0.9391
\\

  & \textcolor{red}{139.37\%} &\textcolor{red}{69.95\%} &\textcolor{red}{3.06\%} &\textcolor{red}{65.16\%} &\textcolor{red}{38.77\%} &\textcolor{red}{2.27\%} &\textcolor{red}{83.07\%} &\textcolor{red}{35.23\%} &\textcolor{red}{3.13\%} 

& \textcolor{red}{96.25\%} &\textcolor{red}{29.37\%} &\textcolor{red}{1.34\%} &\textcolor{red}{134.75\%} &\textcolor{red}{20.71\%} &\textcolor{red}{1.94\%} &\textcolor{red}{142.39\%} &\textcolor{red}{17.10\%} &\textcolor{red}{2.88\%}
\\
\hline

\multirow{2}{*}{EdgeConnect}  &7.0074 &0.0921 &0.9124 &6.1678 &0.0919 &0.9033 &69196 &0.1107 &0.8783 &1.3542 &0.1110 &0.9347 &3.6796 &0.1347 &0.8720 &8.5293 &0.1588 &0.8492 \\

  & \textcolor{red}{49.29\%} &\textcolor{red}{20.87\%} &\textcolor{red}{1.33\%} &\textcolor{red}{24.34\%} &\textcolor{red}{19.97\%} &\textcolor{red}{1.41\%} &\textcolor{red}{27.78\%} &\textcolor{red}{23.41\%} &\textcolor{red}{2.10\%}

&\textcolor{red}{149.12\%} &\textcolor{red}{37.55\%} &\textcolor{darkgreen}{1.77\%} &\textcolor{red}{218.44\%} &\textcolor{red}{25.16\%} &\textcolor{red}{1.58\%} &\textcolor{red}{293.00\%} &\textcolor{red}{20.67\%} &\textcolor{red}{1.71\%} \\\hline 


      
\end{tabular}
 }
\end{center}

%\vspace{-5mm}
\end{table*}
